Certified Robust Control under Adversarial Perturbations

Autonomous systems increasingly rely on machine learning techniques to transform high-dimensional raw inputs into predictions that are then used for decision-making and control. However, it is often easy to maliciously manipulate such inputs and, as a result, predictions. While effective techniques have been proposed to certify the robustness of predictions to adversarial input perturbations, such techniques have been disembodied from control systems that make downstream use of the predictions. We propose the first approach for composing robustness certification of predictions with respect to raw input perturbations with robust control to obtain certified robustness of control to adversarial input perturbations. We use a case study of adaptive vehicle control to illustrate our approach and show the value of the resulting end-to-end certificates through extensive experiments.

==> Notation.tex <==
\section{Notation}
Notations:
\begin{itemize}
    \item $Y$: the labels set. 
    \item $A = \{a_1, a_2, \cdots, a_n \}$ is the interested label sets. 
\end{itemize}

==> contribution.tex <==


\section{Contribution}
\begin{enumerate}
    \item An end to end vision based certified robust control system.
    \item Optimize between robustness and utility (velocity)
    \item Unify terminology.
    \begin{itemize}
        \item The perception part: For an input frame, the perception model outputs a range of road friction, as well as a certified radius. 
        \begin{enumerate}
            \item $\bold{y} = \bold{f}(\bold{x})$, the perception model $\bold{f}$ gives a prediction $\bold{y}$ for the unmodified input frame $\bold{x}$.
            \item Based on $\bold{y}$, we will get a range $\bold{h}(\bold{y})$ determined by the utility function. For example, if the prediction of the road friction is 5.4 in an unmodified environment, then the range might be [5.4, 6.0]. 
            (Based on the safety and efficiency bound.)
            \item The certified radius: The prediction of the perception model will be constant, or in the road friction range, to any noise or adversarial examples that defined within the radius. 
        \end{enumerate}
        \item The control part needs to know the following:
        \begin{itemize}
            \item $\hat{C}_f$: Nominal cornering stiffness of front tire. We can choose most likely value for the nominal cornering stiffness. If you provide range of cornering stiffness only, we can use its center point for the nominal value.
            \item $\hat{C}_r$: Nominal cornering stiffness of rear tire (we can assume $\hat{C}_r=\hat{C}_f$)
            \item $C_f \in [\underline{C}_f,\bar{C}_f]$: range of uncertainty, where $\underline{C}$, $\bar{C}$ imply min, max, respectively.
            \item $C_r\in [\underline{C}_r,\bar{C}_r]$: we can assume $[\underline{C}_f,\bar{C}_f]=[\underline{C}_r,\bar{C}_r]$ again.
        \end{itemize}
    \end{itemize}
\end{enumerate}

==> end2end.tex <==

\subsection{A Case Study}

% We adopt the randomized smoothing techniques \cite{cohen2019certified,chiang2020detection} to construct a certified robust road condition classification model and a certified robust road friction model. In the classification case, the robust road condition classification model is robust against certified malicious attacks, and predicts a road condition class, for example, snow or rain. Then this predicted label is mapped to an interval of cornering stiffness by some physics model. 
% In the regression case, we will show that the predicted road friction of the robust regression model is guaranteed to be within an interval. 
% Given a non-perturbed driving frame, if the non-robust model makes correct decision, we proves the certified road friction interval from its corresponding robust (smoothed) model includes the ground truth cornering stiffness. The $\LL_1$ adaptive controller then makes safe driving commands basing on this certified road friction interval.


% If the constraint in \label{app:C}, i.e., the road friction interval contains the ground truth road friction, the  is satisfied, 

% The 
% takes a road friction interval as an input, 
% stable control. 

If the road friction interval contains the ground truth road friction, 
the $\LL_1$ adaptive controller guarantees transient and steady-state performance with respect to the reference system and design system. 
Given the design parameters chosen in Section~\ref{sec:L1}, 
we analyze the performance of the driving system. 
%we can analyze the performance bounds $\|x_{ref}-x_{des}\|_{\LL_{\infty}}$ and $\|u_{ref}-u_{des}\|_{\LL_{\infty}}$.

\begin{theorem} (Guaranteed controller performance)
If~\eqref{app:C} holds, then there exist positive constants $c_1$ and $c_2$ such that
\begin{align}
    \|x_{des}-x(t)\|_{\LL_{\infty}} \leq c_1, \quad
    \|u_{des}-u(t)\|_{\LL_{\infty}} \leq c_2
    \label{eq:the21}
\end{align}
for $\forall t$. Furthermore, it holds that
\begin{align}
    \lim_{t \rightarrow \infty}\|x_{ref}-x(t)\|=0, \quad \lim_{t \rightarrow \infty}\|u_{ref}-u(t)\|=0.
    \label{eq:the22}
\end{align}
\label{the2}
\end{theorem}
\begin{proof}
The controller with the system satisfy $\LL_1$ adaptive control assumptions, and thus by Theorem 2.1.1 and Lemma 2.1.4 in~\cite{hovakimyan2010L1}, the statement holds true. Constant bounds $c_1$ and $c_2$ are found in~\cite{hovakimyan2010L1}.
\end{proof}

Finally, we integrate the robust perception model and the robust controller together. 
We start with looking at the road condition classification problem. 
The classification model $f_c$ takes the driving frame as input and outputs a road condition class, e.g., snow or asphalt. 
This predicted road condition class is then mapped to a road friction interval by the function $\zeta$. 
This road friction interval is the input to robust control algorithm $U$.

\begin{definition} (Certified Robust \emph{Perception-Control} System (classification))
Recall $f_c : \mathbb{R}^d \rightarrow \mathcal{C}$ is a classification function, 
and
$g$ is the smoothed function of $f_c$ defined in Lemma
\ref{lemma:classification},
$S$ defines a \emph{safety} set for a class.
$\zeta$ maps a set of class to an interval $\mathcal{I}_c$
The robust perception-control system $\mathcal{W}_c$ is defined as,
\begin{align}
    \mathcal{W}_c = \mathcal{U} \circ \zeta \circ S \circ g
\end{align}
\end{definition}

\begin{corollary} (Stability of $\mathcal{W}_c$) 
Recall lemma \ref{lemma:classification},
$a = \argmax_{a \in \mathcal{Y}} g(z)$
and
$b = \argmax_{b \in {\mathcal{Y} \setminus S(a)}} g(z)$. 
Let $(x_{des},u_{des})=\mathcal{W}_c(z_t+\delta)$.
If $\norm{\delta}_{2}\leq\frac{\sigma}{2}(\Phi^{-1}(\underline{\mathbb{P}_a})-\Phi^{-1}(\overline{\mathbb{P}_{b})})$,
then $x_{des}$ and $u_{des}$ satisfy the inequalities \ref{eq:the21} and equations \ref{eq:the22}. 
\end{corollary}

\begin{hproof}
Given an input image $z$ and its ground truth class $c^t$,
we consider the case where the prediction of the non-robust model is within $S(c^t)$, $f_c(x) \in S(c^t)$.  
From Lemma \ref{lemma:classification}, we know
$g(z+\delta) \in S(c^t)$ such that $\norm{\delta}_{2}\leq\frac{\sigma}{2}(\Phi^{-1}(\underline{\mathbb{P}_a})-\Phi^{-1}(\overline{\mathbb{P}_{b})})$
Thus $\zeta \circ S(c^t)$ contains the ground truth road friction.
Combining this observation with the statements in ~\eqref{app:C}, 
we know that equations in Theorem ~\eqref{eq:the22} holds.  
\end{hproof}


Finally, let's discuss the case where the perception model is a regression function $h : \mathbb{R}^d \rightarrow R$. 
The input of the robust perception model $h$ is a driving frame, the output is a certified road friction interval. 

\begin{definition}(
Certified Robust perception-control system (regression))
Recall $h : \mathbb{R}^d \rightarrow R$ is 
a robust smoothing regression function, 
and its output is a certified interval $\mathcal{I}_p$. 
The robust control algorithm is $\mathcal{U}$. 
Then the certificated robust perception-control
system $\mathcal{W}_r$, where the perception model is a regression model, is defined as:
\begin{align}
    \mathcal{W}_r = \mathcal{U} \circ h
\end{align}
\end{definition}

% Recall $h_p$ is the $p$ percentile smoothed function of road friction regression $h$,
% and $\underline{C} = \underline{h}_{\underline{p}}(x), 
% \overline{C} = \overline{h}_{\overline{p}}(x)$. 

% In the road friction regression problem,
% the input to the \emph{control system} is given by the smoothed regression model $h_p$. 
% From lemma .
 
% given any perturbed image as input, 
% the prediction of the smoothed regression model is within an interval. This interval contains the truth 
% The perception model predicts 


\begin{corollary} (Stability of $\mathcal{W}_r$) 
Given any perturbation $\delta$ that is bounded by $l2$ norm, certified robust \emph{perception-control} system $\mathcal{W}_r$ guarantees the equations \eqref{eq:the22} in Theorem \ref{the2}. 
\end{corollary}

\begin{hproof}
In the malicious environment, 
the input image is perturbed to $z+\delta$. 
A defender uses the smooth function $h_p$ predict the road friction. 
Recall Lemma \ref{lemma:regression}, $h_p(z+\delta)$ is bounded by $h_{\underline{p}}(z)$ and $h_{\overline{p}}(z)$. 
Let $y_t$ be the ground truth label. 
\cite{salman2019provably} shows that 
the Gaussian smoothing function $h(z)$ of $f(z)$ is $\sqrt{\frac{2}{\pi}}$\emph{-Lipschitz} continuous,  
Therefore if the prediction without any attack is close to the ground truth, 
i.e., $\norm{f(z)-y^t}$ is bounded by some small number,
$y^t \in [h_{\underline{p}}(z),h_{\overline{p}}(z)]$. 
Combining this observation with the statements in ~\eqref{app:C}, 
we know that equations in Theorem ~\eqref{eq:the22} holds.  
\end{hproof}









%\TODO : Potential theoretical contribution: Velocity differences based on certification range (e.g., strict interval, completely different intervals)

%\TODO : Theoretical guarantee for lateral and longitudinal stability







==> others.tex <==
\section{Potential Interesting Problems}

\subsection{A Sequence of Frames}

==> structure.tex <==





==> theories2.tex <==



Notations:
\begin{itemize}
    \item $Y$: the labels set. 
    \item $A = \{a_1, a_2, \cdots, a_n \}$ is the interested label sets. 
    \item $C = Y \setminus A$.
\end{itemize}



% \begin{proof}
% Add the proof. 
% % For any $x'$ within this ball, we have 
% % \[
% % |{F(x')_R - F(x)_R}| = |F(x')_R - (p_{a_1} + p_{a_2} + p_{a_3} )| \leq L \norm{x' - x} < \frac{1}{2}((p_{a_1} + p_{a_2} + p_{a_3})
% % \]
% \end{proof}

\begin{lemma}
Let $\sigma>0$, $h :  {\rm I\!R }^{d} \rightarrow \ [0,1] $ be arbitrary, and $H = h * \mathcal{N}(0,\sigma^{2}*I)$, Then the function $\Phi^{-1}(H(x))$ is $\frac{1}{\sigma}$-Lipschitz.   
\label{lemma:probBound}
\end{lemma}

\begin{proof}
From \cite{Salman2019ProvablyRD}. 
\end{proof}


\begin{lemma}
Let $f : {\rm I\!R^{d} } \rightarrow \mathcal{P(Y)}$ be any soft classifier, let $\sigma > 0$, and let $F$ be its associated smooth classifier. Let 

\[
a_1 = \argmax_{y \in \mathcal{Y}} F(x)_{y} \qquad and \qquad A = \{a_1, a_2, \cdots, a_n\}. 
\]

% \[
% c = \argmax_{y \in \mathcal{C}} F(x)_{y}. 
% \]

% \textcolor{blue}{What is the relationship between any label in $\{a_2, a_3, \cdots,a_n\}$ and $a_1$.} 

Then we have that $\argmax_{y\in\mathcal{Y}}F(x')  \subset A$ for all $x'$ satisfying 
$\norm{x' - x}_{2} \leq \frac{1}{2L}(\Phi^{-1}(\sum_i p_{a_i}) - ?)$

\label{lemma:multiClass}
\end{lemma}

\begin{proof}
\textcolor{red}{With Lemma \ref{lemma:probBound}, we have 
\[
\norm{\Phi^{-1}(F(x)_A) - \Phi^{-1}(F(x+\delta)_A)} \leq \frac{1}{\sigma}\norm{\delta}_2
\]
}
\[
\Phi^{-1}(F(x)_A) -  \norm{\delta}_2 \leq \Phi^{-1}(F(x+\delta)_A)
\]

For an adversary $\delta$, where $B$ is a set of labels, $s.t. \quad B \bigcap A = \emptyset$, (\textcolor{red}{also should be the second most likely set})
This leading to $F_b(x+\delta) \ge F_a(x+\delta) $,
\[
\Phi^{-1}(F_B(x+\delta)) \ge \Phi^{-1}(F_A(x+\delta))
\]
\[
\Phi^{-1}(F_b(x+\delta)) \leq \Phi^{-1}(F_b(x)) + \norm{\delta}_2
\]
\[
\norm{\delta}_2 \ge \frac{\sigma}{2}(\Phi^{-1}(\sum_i p_{a_i}) - \Phi^{-1}(F_B(x)) )
\]

\end{proof}





% \begin{theorem}
% Radius $\frac{\sigma}{2}(\sum_i \Phi^{-1}(p_{a_i}) - \Phi^{-1}(p_b))$
% \label{thm:multiClass}
% \end{theorem}

% \begin{proof}
% Combining Lemma \ref{lemma:multiClass} and Lemma \ref{lemma:probBound} yields Theorem \ref{thm:multiClass}
% \end{proof}

% In the case, we only certify the exact original class, (The original theorem of randomized smoothing:)
\begin{theorem}
Let $F :  {\rm I\!R }^{d} \rightarrow \ \mathcal{P(Y)} $ be any soft classifier, let $\sigma > 0$, and let $G$ be its associated smooth classifier. Let 
\[
a = \argmax_{y \in \mathcal{Y}} G(x)_y \qquad and \qquad b = \argmax_{y \in \mathcal{Y} \not\in \{y*\} } G(x)_y
\]
be the two most likely classes for x according to G. Then we have that $\argmax_{y\in \mathcal{Y}} G(x')_y = a$ for all $x'$ satisfying 

\[
\norm{x'-x}_2 \leq \frac{\sigma}{2}( \Phi^{-1}(p_a) - \Phi^{-1}(p_b)
)
\]

\label{thm:twoClass}
\end{theorem}






% \begin{theorem}[Pythagorean theorem]
% \label{pythagorean}
% This is a theorema about right triangles and can be summarised in the next 
% equation 
% \[ x^2 + y^2 = z^2 \]
% \end{theorem}

% And a consequence of theorem \ref{pythagorean} is the statement in the next 
% corollary.

% \begin{corollary}
% There's no right rectangle whose sides measure 3cm, 4cm, and 6cm.
% \end{corollary}

% You can reference theorems such as \ref{pythagorean} when a label is assigned.

% \begin{lemma}
% Given two line segments whose lengths are $a$ and $b$ respectively there is a 
% real number $r$ such that $b=ra$.
% \end{lemma}
